Spectral extended finite element method for band structure calculations in phononic crystals

In this paper, we compute the band structure of one- and two-dimensional phononic composites using the extended finite element method (X-FEM) on structured higher-order (spectral) finite element meshes. On using partition-of-unity enrichment in finite element analysis, the X-FEM permits use of structured finite element meshes that do not conform to the geometry of holes and inclusions. This eliminates the need for remeshing in phononic shape optimization and topology optimization studies. In two dimensions, we adopt rational B{\'e}zier representation of curved (circular) geometries, and construct suitable material enrichment functions to model two-phase composites. A Bloch-formulation of the elastodynamic phononic eigenproblem is adopted. Efficient computation of weak form integrals with polynomial integrands is realized via the homogeneous numerical integration scheme -- a method that uses Euler's homogeneous function theorem and Stokes's theorem to reduce integration to the boundary of the domain. Ghost penalty stabilization is used on finite elements that are cut by a hole. Band structure calculations on perforated (circular holes, elliptical holes, and holes defined as a level set) materials as well as on two-phase phononic crystals are presented that affirm the sound accuracy and optimal convergence of the method on structured, higher-order spectral finite element meshes. Several numerical examples demonstrate the advantages of $p$-refinement made possible by the spectral extended finite element method. In these examples, fourth-order spectral extended finite elements deliver $\mathcal{O}(10^{-8})$ accuracy in frequency calculations with more than thirty-fold fewer degrees-of-freedom when compared to quadratic finite elements.

==> phononics-1D.tex <==
\subsection{One-dimensional two-phase phononic crystal}

\subsubsection{Phononic eigenvalues}
We consider a two-phase composite in one dimension. The unit cell domain is
$\Omega = (0,a)$ with length $a := h_1 + h_2$. The interface is located at $x =
h := h_1$. The Young's modulus and density of phase 1 are $E_1$ and $\rho_1$ and
that of phase 2 are $E_2$ and $\rho_2$, respectively.

For the numerical computations, we set $h_1 = h_2 = 0.003$ mm and $\rho_1 =
\rho_2 = 3000$ kg/$\textrm{m}^3$. The Young's modulus of phase 1 is $E_1 = 11$
GPa. To assess the performance of spectral finite elements for sharp contrasts
in Young's modulus, $E_2$ is chosen such that $E_1/E_2$ varies from $10^{-3}$ to
$10^{3}$. In the irreducible Brillouin zone, we consider $0 \le Q \le 0.5$,
where $Q := ka/(2\pi)$ and $k$ is the wavevector. We choose $Q = 0.25$ and
compare the relative error in the frequency $f$ ($\omega = 2 \pi f$) using
spectral FE and Rayleigh quotient using PWE. For spectral FE, we use 20
eight-order spectral elements (160 DOFs), whereas for Rayleigh quotient we use
300 plane waves to obtain the reference solutions.

The finite element solution is obtained using 2 eight-order spectral elements,
and has 16 DOFs. A 10-point Gauss quadrature rule is used. The Rayleigh quotient
solution using planewaves is computed with 100 DOFs. In~\fref{fig:1dcomposite},
we compare the relative error in the frequency with spectral FE and Rayleigh
quotient for the five lowest eigenvalues. We observe that spectral FE delivers
much better accuracy than Rayleigh quotient with far fewer DOFs. For
discontinuous material properties, spectral FE can have striking advantages over
Rayleigh quotient.
%
\begin{figure}
\centering
  \begin{subfigure}{0.3\textwidth}
     \includegraphics[width=\textwidth]{spectral1D-123.pdf}
     \caption{}\label{fig:1dcomposite-a}
  \end{subfigure}\hfill
  \qquad
  \begin{subfigure}{0.3\textwidth}
     \includegraphics[width=\textwidth]{spectral1D-45.pdf}
     \caption{}\label{fig:1dcomposite-b}
  \end{subfigure}\hfill
  \begin{subfigure}{0.35\textwidth}
     \includegraphics[width=\textwidth]{Rayleigh_Relative_err_M_semilogx.pdf}
     \caption{}\label{fig:1dcomposite-c}
  \end{subfigure}
\caption{Two-phase one-dimensional phononic crystal.
         Relative error in the frequencies at $Q = 0.25$ for the five 
         lowest eigenvalues. (a),(b) Eight-order
         spectral FE (16 DOFs).  Lowest three eigenvalues are shown in
         (a) and fourth and fifth eigenvalues are plotted in (b). 
         Errors in the lowest two eigenvalues
         are close to machine precision; and (c) Rayleigh quotient using PWE (100 DOFs).}
         \label{fig:1dcomposite}
\end{figure}

\subsubsection{Band gap maximization for PC design}

Use X-FEM to solve a 1-D band gap maximization problem to design a PC.

